A multi-instrument non-parametric reconstruction of the electron pressure profile in the galaxy cluster CLJ1226.9+3332

Context: In the past decade, sensitive, resolved Sunyaev-Zel'dovich (SZ) studies of galaxy clusters have become common. Whereas many previous SZ studies have parameterized the pressure profiles of galaxy clusters, non-parametric reconstructions will provide insights into the thermodynamic state of the intracluster medium (ICM). Aims: We seek to recover the non-parametric pressure profiles of the high redshift ($z=0.89$) galaxy cluster CLJ 1226.9+3332 as inferred from SZ data from the MUSTANG, NIKA, Bolocam, and Planck instruments, which all probe different angular scales. Methods: Our non-parametric algorithm makes use of logarithmic interpolation, which under the assumption of ellipsoidal symmetry is analytically integrable. For MUSTANG, NIKA, and Bolocam we derive a non-parametric pressure profile independently and find good agreement among the instruments. In particular, we find that the non-parametric profiles are consistent with a fitted gNFW profile. Given the ability of Planck to constrain the total signal, we include a prior on the integrated Compton Y parameter as determined by Planck. Results: For a given instrument, constraints on the pressure profile diminish rapidly beyond the field of view. The overlap in spatial scales probed by these four datasets is therefore critical in checking for consistency between instruments. By using multiple instruments, our analysis of CLJ 1226.9+3332 covers a large radial range, from the central regions to the cluster outskirts: $0.05 R_{500} < r < 1.1 R_{500}$. This is a wider range of spatial scales than is typical recovered by SZ instruments. Similar analyses will be possible with the new generation of SZ instruments such as NIKA2 and MUSTANG2.

==> table_pressure_profile_results.tex <==
%\begin{landscape}

\begin{deluxetable*}{l|lllllllllll}
\tabletypesize{\scriptsize}
\tablecolumns{12}
\tablewidth{\columnwidth} 
\tablecaption{Summary of Fitted Pressure Profiles \label{tbl:pressure_profile_results}}
\tablehead{
\colhead{Cluster} & \colhead{$R_{500}^a$} & \colhead{$Y_{sph}(R_{500})$} & \colhead{$P_{500}^a$} & 
        \colhead{$P_0$} & \colhead{$C_{500}$} & \colhead{$\alpha$} & \colhead{$\beta$} & \colhead{$\gamma$} & 
                  \colhead{$k$} & \colhead{$\tilde{\chi}^2$} &  \colhead{d.o.f.}        \\ 
      & \colhead{(Mpc)} & \colhead{($10^{-5}$ Mpc$^2$)} & \colhead{$10^{-3}$ keV cm$^{-3}$} & \colhead{}  & 
      \colhead{} & \colhead{}  & \colhead{}  & \colhead{}  &   \colhead{}    
}
\startdata
Abell 1835 & 1.49 & $22.50_{-4.49}^{+4.12}$ &  5.94 & $2.15 \pm 0.07$ & $0.77_{-0.17}^{+0.23}$ & 
1.05 & 5.49 & $0.78_{-0.13}^{+0.12}$ & 1.08 & 0.99 & 12880   \\ 
Abell 611  & 1.24 &  $8.14_{-2.21}^{+3.68}$ &  4.45 & $35.43 \pm 2.46$ & $2.00_{-0.30}^{+0.40}$ & 
1.05 & 5.49 & $0.00^{+0.15}$ & 0.96 & 1.02 & 12882   \\ 
MACS 1115  & 1.28 & $20.53_{-3.52}^{+3.84}$ &  5.45 & $0.67 \pm 0.04$ & $0.35_{-0.10}^{+0.15}$ & 
1.05 & 5.49 & $0.87_{-0.27}^{+0.18}$ & 1.11 & 1.04 & 12875   \\ 
MACS 0429  & 1.10 & $19.85_{-3.74}^{+4.00}$ &  4.48 & $11.01 \pm 0.77$ & $0.59_{-0.09}^{+0.11}$ & 
1.05 & 5.49 & $0.00^{+0.15}$ & 1.00 & 1.03 & 12875   \\ 
MACS 1206  & 1.61 & $43.24_{-8.27}^{+8.19}$ & 10.59 & $2.39 \pm 0.10$ & $0.74_{-0.14}^{+0.16}$ & 
1.05 & 5.49 & $0.51_{-0.16}^{+0.14}$ & 1.09 & 1.01 & 12874   \\ 
MACS 0329  & 1.19 & $12.91_{-2.37}^{+2.93}$ &  5.93 & $9.30 \pm 0.50$ & $1.18_{-0.28}^{+0.72}$ & 
1.05 & 5.49 & $0.41_{-0.41}^{+0.19}$ & 1.03 & 0.99 & 12876   \\ 
RXJ1347    & 1.67 & $37.69_{-5.11}^{+5.78}$ & 11.71 & $3.24 \pm 0.08$ & $1.18_{-0.48}^{+1.02}$ & 
1.05 & 5.49 & $0.80_{-0.70}^{+0.30}$ & 1.15 & 0.99 & 12880   \\ 
MACS 1311  & 0.93 & $10.16_{-1.73}^{+1.79}$ &  3.99 & $2.75 \pm 0.22$ & $0.35_{-0.05}^{+0.15}$ & 
1.05 & 5.49 & $0.41_{-0.41}^{+0.34}$ & 0.98 & 1.00 & 12881   \\ 
MACS 1423  & 1.09 &  $8.47_{-2.07}^{+2.53}$ &  6.12 & $22.39 \pm 1.71$ & $1.58_{-0.48}^{+0.22}$ & 
1.05 & 5.49 & $0.00^{+0.35}$ & 1.04 & 0.98 & 12876   \\ 
MACS 1149  & 1.53 & $42.77_{-5.67}^{+4.99}$ & 12.28 & $5.50 \pm 0.25$ & $0.83_{-0.03}^{+0.07}$ & 
1.05 & 5.49 & $0.00^{+0.05}$ & 0.87 & 1.00 & 13584   \\ 
MACS 0717  & 1.69 & $43.44_{-8.00}^{+9.28}$ & 14.90 & $21.28 \pm 0.68$ & $1.97_{-0.37}^{+0.53}$ & 
1.05 & 5.49 & $0.00^{+0.25}$ & 0.48 & 1.04 & 12876   \\ 
MACS 0647  & 1.26 & $26.22_{-4.72}^{+5.37}$ &  9.23 & $2.78 \pm 0.11$  & $0.70_{-0.20}^{+0.30}$ & 
1.05 & 5.49 & $0.60_{-0.20}^{+0.15}$ & 1.14 & 1.01 & 12876   \\ 
MACS 0744  & 1.26 & $12.59_{-2.29}^{+3.18}$ & 11.99 & $13.15 \pm 0.81$ & $1.71_{-0.21}^{+0.29}$ & 
1.05 & 5.49 & $0.00^{+0.15}$ & 0.90 & 1.02 & 12875   \\ 
CLJ1226    & 1.00 &  $9.03_{-1.60}^{+2.03}$ & 11.84 & $19.29 \pm 1.25$ & $1.90_{-0.50}^{+0.60}$ & 
1.05 & 5.49 & $0.29_{-0.29}^{+0.36}$ & 0.92 & 1.03 & 12875   \\ 
\hline
All          &  --    &  --    &  --    &  $7.94  \pm 0.10$ & $1.3_{-0.1}^{+0.1}$ & 1.05 & 5.49 & $0.3_{-0.1}^{+0.1}$ & -- & -- & -- \\ 
Cool Core    &  --    &  --    &  --    &  $3.55  \pm 0.06$ & $0.9_{-0.1}^{+0.1}$ & 1.05 & 5.49 & $0.6_{-0.1}^{+0.1}$ & -- & -- & -- \\
Disturbed    &  --    &  --    &  --    &  $12.56 \pm 0.29$ & $1.5_{-0.2}^{+0.1}$ & 1.05 & 5.49 & $0.0^{+0.1}$       & -- & -- & -- \\ 
Well behaved &  --    &  --    &  --    &  $5.34 \pm 0.08$ & $1.2_{-0.1}^{+0.1}$ & 1.05 & 5.49 & $0.5_{-0.1}^{+0.1}$  & -- & -- & -- \\ 
\hline
All (A10)    &  --    &  --    &  --    &  $8.403 h_{70}^{-3/2}$ & 1.177 & 1.0510 & 5.4905 & 0.3081 & -- & -- & -- \\
Cool core (A10) &  --    &  --    &  --    &  $3.249 h_{70}^{-3/2}$ & 1.128 & 1.2223 & 5.4905 & 0.7736 & -- & -- & -- \\
Disturbed (A10) &  --    &  --    &  --    &  $3.202 h_{70}^{-3/2}$ & 1.083 & 1.4063 & 5.4905 & 0.3798 & -- & -- & --
\enddata
\tablecomments{Results from our pressure profile analysis. $Y_{sph}$ is calculated using the tabulated value of $R_{500}$.
    $^a$Values of $R_{500}$ and $P_{500}$ are taken from \citet{sayers2013}. We have assumed A10 values of $\alpha$ and $\beta$.
    The findings from A10 are reproduced in the last three rows. The $h_{70}$ dependence is included for explicit replication
    of A10 results; all $P_0$ values have this dependence (the assumed cosmologies are the same).}
\end{deluxetable*}

%\end{landscape}

